A Survey on the Explainability of Supervised Machine Learning

Predictions obtained by, e.g., artificial neural networks have a high accuracy but humans often perceive the models as black boxes. Insights about the decision making are mostly opaque for humans. Particularly understanding the decision making in highly sensitive areas such as healthcare or fifinance, is of paramount importance. The decision-making behind the black boxes requires it to be more transparent, accountable, and understandable for humans. This survey paper provides essential definitions, an overview of the different principles and methodologies of explainable Supervised Machine Learning (SML). We conduct a state-of-the-art survey that reviews past and recent explainable SML approaches and classifies them according to the introduced definitions. Finally, we illustrate principles by means of an explanatory case study and discuss important future directions.

==> math.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   Identification
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\NeedsTeXFormat{LaTeX2e}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   Preliminary declarations
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\RequirePackage{bm} % correct bold symbols, like \bm
\RequirePackage{amsmath}
\RequirePackage{amsfonts}
\RequirePackage{amssymb}
%\RequirePackage{mathrsfs}
%\RequirePackage{dsfont} % double stroke symbols like IR
%\RequirePackage[single]{accents} % own accents 
%\RequirePackage{exscale} % Scaling of Math Symbols?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   Options
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   More declarations
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%------------------------------------------------------------
% Mathematical Formulae
%------------------------------------------------------------
\newcommand{\rv}[1]{\ensuremath{{\boldsymbol{#1}}}}
\renewcommand{\vec}[1]{\ensuremath{{\underline{#1}}}}
\newcommand{\rvec}[1]{\ensuremath{{\boldsymbol{\underline{#1}}}}}
\newcommand{\mat}[1]{{\ensuremath{{\mathbf{#1}}}}}

\newcommand{\SquareRoot}[1]{{\mbox{\bfseries\sffamily #1}}}
\newcommand{\intndim}{\ds\int_{-\infty}^\infty \dots \int_{-\infty}^\infty}
\newcommand{\Eye}{\mat{I}}

% operators (in alphabetical order):
\renewcommand{\arg}{\operatorname*{arg}}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\argmin}[1]{\mathop{\mathrm{arg}\; \min_{#1}}}
\newcommand{\argmax}[1]{\mathop{\mathrm{arg}\; \max_{#1}}}
\def\DEF{\triangleq} % definition symbol
\DeclareMathOperator{\col}{col}
\newcommand{\dd}{\operatorname{d}\!}
%\def\d{\ensuremath{\operatorname{d}}} % for \int f(x)\d x or \d y / \d y
%\renewcommand{\d}{\ensuremath{\text{d}}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\E}{E}
\DeclareMathOperator{\MI}{I}
\DeclareMathOperator{\ENT}{H}
\DeclareMathOperator{\Proj}{proj}
\renewcommand{\Pr}{\operatorname{P}} 
\DeclareMathOperator{\rang}{rang}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\jj}{j}% complex unit
\DeclareMathOperator{\rect}{rect}
\def\T{^\mathrm{T}} % transpose
\def\inv{^{-1}} % inverse
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator*{\Var}{Var} 
\renewcommand{\arctan}{\operatorname{arctan}}
\newcommand{\atann}{\operatorname{arctan2}}
%\DeclareMathOperator{\atan}{atan}
\def\atan2{\operatorname{atan2}}
\DeclareMathOperator{\pot}{pot}
\DeclareMathOperator{\sign}{sign}

\newcommand{\FromTo}[2]{$#1 = 1,\, \ldots,\, #2$}
\newcommand{\LMInd}{{\operatorname{LM}}}

%---------------------------------------------------------------------
% Abbreviations
%---------------------------------------------------------------------

\def\({\left(}
\def\){\right)}
\def\[{\left[}
\def\]{\right]}

\newcommand{\ds}{\displaystyle}
\newcommand{\ns}{\textstyle}

\newcommand{\NewB}{\ensuremath{\mathds{R}}}
\newcommand{\NewC}{\ensuremath{\mathds{C}}}
\newcommand{\NewN}{\ensuremath{\mathds{N}}}
\newcommand{\NewQ}{\ensuremath{\mathds{Q}}}
\newcommand{\NewR}{\ensuremath{\mathds{R}}}
\newcommand{\NewZ}{\ensuremath{\mathds{Z}}}
\newcommand{\IR}{\NewR}
\newcommand{\IN}{\NewN}
\newcommand{\IZ}{\NewZ}
\newcommand{\IC}{\NewC}

\newcommand{\Gauss}{{\mathcal{N}}}

\setcounter{MaxMatrixCols}{20} %Fuer ams umgebung


%--------------------------------------------------------------------------
%Einheiten mit korrekten Leerzeichen
%Usage: \Meter{\micro}{10} results $10\mu m$ 
\newcommand{\Meter}[2][]{\unit{#2}#1\meter} 
\newcommand{\Volt}[2][]{\unit{#2}#1\volt} 
\newcommand{\Hertz}[2][]{\unit{#2}#1\hertz} 
\newcommand{\Second}[2][]{\unit{#2}#1\second} 
\newcommand{\Pascal}[2][]{\unit{#2}#1\pascal} 
\newcommand{\Euro}[2][]{\unit{#2}#1\euro}

\newcommand{\nm}[1] {\Meter[\nano]{#1}}
\newcommand{\mum}[1]{\Meter[\micro]{#1}}
\newcommand{\mm}[1] {\Meter[\milli]{#1}}
\newcommand{\cm}[1] {\Meter[\centi]{#1}}
\newcommand{\mV}[1] {\Volt[\milli]{#1}}
\newcommand{\ms}[1] {\Second[\milli]{#1}}
\newcommand{\KHz}[1] {\Hertz[\kilo]{#1}}


%------------------------ Random variables ---------------------------
\def\u{\rv u}
\def\v{\rv v}
\def\w{\rv w}
\def\x{\rv x}
\def\y{\rv y}
\def\z{\rv z}

%---------------------------- Vectors --------------------------------
\def\vdel{\vec \delta}
\def\veta{\vec \eta}
\def\vOmega{\vec \Omega}
\def\vsig{\vec \sigma}
\def\va{\vec a}
\def\vb{\vec b}
\def\vc{\vec c}
\def\vd{\vec d}
\def\ve{\vec e}
\def\vf{\vec f}
\def\vg{\vec g}
\def\vh{\vec h}
\def\vmu{\vec \mu}
\def\vp{\vec p}
\def\vs{\vec s}
\def\vpi{\vec \pi}
\def\vthe{\vec \theta}
\def\vu{\vec u}
\def\vv{\vec v}
\def\vw{\vec w}
\def\vx{\vec x}
\def\vy{\vec y}
\def\vz{\vec z}
\def\vxi{\vec \xi}
\def\vB{\vec B}
\def\vF{\vec F}
\def\vJ{\vec J}
\def\vM{\vec M}
\def\vP{\vec P}
\def\vX{\vec X}

%------------------------- Random vectors ----------------------------
\def\rvn{\rvec n}
\def\rvthe{\rvec \theta}
\def\rvv{\rvec v}
\def\rvw{\rvec w}
\def\rvx{\rvec x}
\def\rvy{\rvec y}
\def\rvz{\rvec z}
\def\rvhz{\rvec{\hat z}}
\def\rvxi{\rvec \xi}
\def\rvX{\rvec X}

%---------------------------- Matrices -------------------------------
\def\A{\mat A}
\def\B{\mat B}
\def\C{\mat C}
\def\D{\mat D}
\def\mE{\mat E}
\def\F{\mat F}
\def\G{\mat G}
\def\H{\mat H}
\def\I{\mat I}
\def\J{\mat J}
\def\K{\mat K}
\def\L{\mat L}
\def\M{\mat M}
\def\P{\mat P}
\def\Q{\mat Q}
\def\R{\mat R}
\def\S{\mat S}
\def\U{\mat U}
\def\V{\mat V}
\def\W{\mat W}
\def\X{\mat X}
% Inverse
\def\iA{\A\inv}
\def\iB{\B\inv}
\def\iC{\C\inv}
\def\iD{\D\inv}
\def\iF{\F\inv}
\def\iM{\M\inv}
\def\iQ{\Q\inv}

%------------------------------ Mean ---------------------------------
\def\ha{\hat a}
\def\hg{\hat g}
\def\hv{\hat v}
\def\hw{\hat w}
\def\hx{\hat x}
\def\hy{\hat y}
\def\hz{\hat z}
\def\hva{\hat{\vec a}}
\def\hvg{\hat{\vec g}}
\def\hvh{\hat{\vec h}}
\def\hvv{\hat{\vec v}}
\def\hvw{\hat{\vec w}}
\def\hvx{\hat{\vec x}}
\def\hvy{\hat{\vec y}}
\def\hvz{\hat{\vec z}}
\def\hvX{\hat{\vec X}}

%------------------------------ Sets ---------------------------------
\def\SA{\mathcal A}
\def\SB{\mathcal B}
\def\SC{\mathcal C}
\def\SD{\mathcal D}
\def\SE{\mathcal E}
\def\SF{\mathcal F}
\def\SG{\mathcal G}
\def\SH{\mathcal H}
\def\SI{\mathcal I}
\def\SL{\mathcal L}
\def\SM{\mathcal M}
\def\SN{\mathcal N}
\def\SO{\mathcal O}
\def\SP{\mathcal P}
\def\SS{\mathcal S}
\def\ST{\mathcal T}
\def\SU{\mathcal U}
\def\SV{\mathcal V}
\def\SW{\mathcal W}
\def\SX{\mathcal X}
\def\SY{\mathcal Y}
\def\SZ{\mathcal Z}

%------------------------------ Misc ---------------------------------
\def\ii{^{(i)}}
\def\ij{^{(j)}}
